A Review of Causal Decision Making

To make effective decisions, it is important to have a thorough understanding of the causal relationships among actions, environments, and outcomes. This review aims to surface three crucial aspects of decision-making through a causal lens: 1) the discovery of causal relationships through causal structure learning, 2) understanding the impacts of these relationships through causal effect learning, and 3) applying the knowledge gained from the first two aspects to support decision making via causal policy learning. Moreover, we identify challenges that hinder the broader utilization of causal decision-making and discuss recent advances in overcoming these challenges. Finally, we provide future research directions to address these challenges and to further enhance the implementation of causal decision-making in practice, with real-world applications illustrated based on the proposed causal decision-making. We aim to offer a comprehensive methodology and practical implementation framework by consolidating various methods in this area into a Python-based collection. URL: https://causaldm.github.io/Causal-Decision-Making.

==> Others/CPLon-lit.tex <==
\begin{enumerate}
    \item \textbf{with prior Causal Information}: There are two common objectives: 1) eliminate the confounding bias for scenario with latent confounders, and 2) sample efficiency, causal explanation and generalization for unconfounded scenarios

    \begin{enumerate}
    \item MAB with single intervention variable
        \begin{enumerate}
            \item eliminating the confounding bias (with unobserved confounders)
            \begin{enumerate}
                \item "Bandits with unobserved confounders: A causal approach": [known causal model (graph+distribution)] a new bandit problem with unobserved confounders using causal graphical representation (the unobserved confounder affect both the action and the outcome). Developing an optimization metric employing both experimental and observational quantities (Is the metric just the effect of the treatment on the treated group?), based on which a Causal TS algorithm is proposed.
                \item "Counterfactual data-fusion for online reinforcement learners": the same motivation as the previous one, but proposed a counterfactual-based decision making. generating counterfactual experiences, then combined the observational, experimental, and counterfactual data to learn the environments in the presence of latent confounder. the assumed causal structure is slightly different from the one assumed in the previous paper, in that there is an intent action $I_t$ between $U_t$ and the policy $\pi_t$.
            \end{enumerate}

        \item sample efficiency
            \begin{enumerate}        
                \item “Regret analysis of bandit problems with causal background knowledge”: [known causal model (graph+distribution)] C-UCB and C-TS, assuming the distribution of parents of the reward for each intervention is known. The proposed method aim to reduce the amount of needed exploration. 
                 \item “Budgeted and non-budgeted causal bandits”: [known causal model (graph+distribution)] $\gamma$-NB-UCB and CRM-NB-ALG for bandits with budget constraint; C-UCB-2 for cases without budget constraint, has the same assumption as the previous one (what is the difference between C-UCB and C-UCB-2 then??????)
            \end{enumerate}
        \end{enumerate}
    \item Contextual bandits
        \begin{enumerate}
            \item sample efficiency (major) \& eliminating confounding bias
            \begin{enumerate}
                \item “Causal contextual bandits with targeted interventions”: standard contextual bandits relies on large sample interactions for each arm, which is costly. Proposed a causal CB to show that even the experiments of each arm is only conducted on a subset of population, the learned reward can still be used to inform an optimal policy regarding the whole population, given casual-side information
                \item \textcolor{red}{“Unifying offline causal inference and online bandit learning for data driven decision”}: utilized the inform from logged data to improve the accuracy. (both context-free and context-dependent, consider the unobserved confounder but not focus on the UC bias): While an AB test may make wrong decisions that harm the user experience and create irreparable damage, offline causal inference is not adaptive to new incoming data. As a result, the authors proposed unifying offline causal inference and online bandit learning. Specifically, they used the counterfactual estimation using offline logged data to assist in warming up the online bandit algorithm.
                \item A Thompson Sampling Approach to Unifying Causal Inference and Bandit Learning: a TS variant as an extension of the above one
                \item “Transfer learning in multi-armed bandit: a causal approach”: transferring knowledge across bandit agents. the first to connect CEL algo and the OPE algo. (also consider the unobserved confounder)
            \end{enumerate}
            \item fairness
            \begin{enumerate}
                \item Achieving Counterfactual Fairness for Causal Bandit: incorporating causal inference into bandits
        
            \end{enumerate}
        \end{enumerate}
    \item SCM-MAB (combinatorial causal bandits): SCM-MAB is a type of MAB, in which there are multiple manipulable intervention variables
        \begin{enumerate}
        \item assume known causal model and no unobserved confounders: somehow show the sample efficiency as the extra causal information can help learn a better policy more quickly
        \begin{enumerate}
            \item “Causal bandits: Learning good interventions via causal inference”: the similar causal bandit problem as the first one. agent can control the allowed actions, estimate the optimal action assuming the arbitrary causal graph was given
            \item “Identifying best interventions through online importance sampling”: considering the same problem as the above one. an efficient successive rejects algorithm with importance sampling, assuming known causal structure.
        \end{enumerate} 
        \item assume known causal structure and no unobserved confounder
        \begin{enumerate}
            \item “Causal bandits with propagating inference”: all previous considered localized interventions. here, propagating inference to propagating throughout the given causal graph.
            \item Causal Bandits for Linear Structural Equation Models
        \end{enumerate}
        \item assume known causal structure and address unobserved confounders
        \begin{enumerate}
            \item “Structural causal bandits: where to intervene?”: explore the possibly optimal minimal intervention set (assuming all observed variables are manipulable)
            \item “Structural causal bandits with non-manipulable variables”: further address the possibility that only a subset of intervention variables is manipulable.
            \item “Characterizing optimal mixed policies: Where to intervene and what to observe”: defined the mixed policy, which determining where to intervene and what to observe. first, find the class of \textbf{non-redundant} policies; then, take the policy with optimal performance. \textbf{The non-redundancy ca help faster the convergence to the optimum}
            \item A Causal Bandit Approach to Learning Good Atomic Interventions in Presence of Unobserved Confounders
            \item Combinatorial causal bandits: provide theoretical analysis compared to the first three papers, which focus on empirical study
        \end{enumerate}
        \end{enumerate}

    \item Semi-parametric bandits + causal inference (Rubins): Semi-parametric Bandits: semi-parametic bandits is proposed to bridge the non-contextual MAB and the contextual bandits, by partially modeling the reward function while leaving some components flexible. However, they easily suffer from increased computational complexity and potentially greater difficulty in obtaining reliable estimates, which an integration with causal inference can help address.
        \begin{enumerate}
        \item optimizing treatment effect instead of reward
            \begin{enumerate}
            \item \textcolor{red}{Contextual Multi-Armed Bandits for Causal Marketing} [single-stage heterogeneous treatment effect estimators + Online Bandits]: The authors estimate and optimize the Conditional Average Treatment Effect (CATE) (i.e., $\tau_{a} = Y(A = a)- Y(A\neq a)$) instead of modeling and maximizing $Y(A = a)$. Primarily, it is driven by the necessity for practical applications, such as advertising, that seek to optimize the return on investment; it is wasteful to send advertisements to customers who already possess a high probability of making a purchase.
            \item An Application of Causal Bandit to Content Optimization
            \item Mitigating Targeting Bias in Content Recommendation with Causal Bandits
            \item \textcolor{red}{Flexible and efficient contextual bandits with heterogeneous treatment effect oracles} [R-learner + contextual bandits]: Unlike a), it is inspired by the finding that 1) genuine reward can contain action-independent redundancy that are irrelevant for decision making and 2) treatment effect estimate bias is no greater than reward model estimation bias under the same model class. It is assumed that $Y(a) = g(x,a) + h(x)$, with $h()$ representing a confounder model and $g()$ representing a true treatment effect model. R-learner is used to estimate $g()$; the likelihood of an action being selected is defined as a function of $g()$; an action with a higher $g(x,a)$ is more likely to be played.
            \end{enumerate}
        \item Experimental Design
            \begin{enumerate}
            \item Synthetically controlled bandits: it used bandits to help traditional synthetic control method saving experimental cost (i.e., if observed reward - estimated reward that would be observed if no treatment for the unit i is negative, then the treatment is discontinued for unit i) 
            \item Multi-armed Bandit Experimental Design: Online Decision-making and Adaptive Inference
            \end{enumerate}
        \end{enumerate}
    \end{enumerate}


    \item \textbf{With no prior causal information}: 
    \begin{enumerate}
    \item causal explanation
    \begin{enumerate}
        \item "Playing against nature: causal discovery for decision making under uncertainty": three cases are considered: 1) the causal model is fully known; 2) only the causal structure is known; 3) the causal model is fully unknown. Focusing on how to acquire causal information from continuous iteration. 

    \end{enumerate}
    \item Causal Bandits with Unknown Graph Structure
    \item Causal Bandits without prior knowledge using separating sets.
    \item Adaptively Exploiting d-Separators with Causal Bandits.
    \item Causal discovery for causal bandits utilizing separating sets
    \item Causal bandits without graph learning
    \end{enumerate}
\end{enumerate}




==> Others/terminology.tex <==
The Relative Strength Index (RSI) is a technical analysis indicator that measures the magnitude of recent price changes to assess overbought or oversold conditions in a security or other asset. It is commonly used to identify potential reversal points in the price of an asset and to help traders make buy or sell decisions.

The RSI is calculated using the average of the gains and losses of an asset over a given period of time. Specifically, the RSI is calculated as the ratio of the average gain to the average loss over the specified time period, multiplied by 100. A high RSI value (above 70) indicates that an asset may be overbought, while a low RSI value (below 30) indicates that it may be oversold.

The RSI is often used in conjunction with other technical analysis indicators, such as moving averages, to provide a more comprehensive view of an asset's price trends and potential entry or exit points for trades. It is also widely used in algorithmic trading systems to help automate the decision-making process.



==> Tables/old_tables.tex <==
\begin{table}
\begin{tabular}{ | m{2cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2cm} | m{2cm} | } 
% \begin{tabular}{ | | |  |  || | } 
  \hline
  Study & State & Action & Reward & Algorithm & Data & Contribution\\ 
  \hline

\citet{ chan2001electronic} & inventory of agent, order imbalance, bid-ask spread and some other market quantity measures functions of price change, etc.)& change in bid and ask prices & a linear combination of profit, inventory risk and
market quality & SARSA and actor-critic algorithm with policy by Boltzmann distribution & Using the simulator of their own & The first to apply RL in market making
\\
\hline


  \citet{Patel2018MM} & Macro agent: historical price data; Market Indicator Features (Price Level, Price Change, Volume Level,
Volume Change, Volatility); Micro agent: time, inventory, end-to-end market information & Macro agent: Buy, sell, or hold the asset; Micro agent: price of limit orders & Macro agent: clipped reward of profit based on decision; Micro agent: profit based on price difference & DQN & Bitcoin data based on historical orderbook& Propose a novel hierarchical decision structure for Market Making Agent\\ 
  \hline
  
  % \citet{Patel2018MM} & Macro agent: historical price data; Market Indicator Features (Price Level, Price Change, Volume Level,Volume Change, Volatility) & Macro agent: Buy, sell, or hold  & Macro agent: clippted reward based on decisionprice information, inventory information, volatility; micro agent: bid-ask information, trade information & Macro agent: Buy, sell, or hold ; micro agent: price of limit order & Macro agent: clippted reward based on decision;  micro agent:  a function of Volume Weighted Average Price& DQN & Bitcoin data based on historical orderbook& Propose a novel hierarchical decision structure for Mmarket Mmaking Aagent\\ 
  % \hline

  
  \citet{Spooner2018MM} & Inventory, active quoting distances, and 
market states (market spread, mid-price move,
book/queue imbalance, signed volume, 
volatility, relative strength index) & Place limit orders at fixed distances to the mid-price; Clear inventory  &  PnL from placing orders and inventory PnL, with asymmetrically dampened reward function designed to encourage making orders rather than profiting from speculation (keeping the inventory) & Q-learning, 
SARSA 
and R-learning & Data from their simulator, which is developed based on historical data & Propose the asymmetrically dampened reward function\\
%   \hline
%   \citet{spooner2020robust} & Current time and the agent's inventory &   Quoted spread and reservation price & Mark-to-market
% (MtM) value of the agent's holding (include both profit of executing orders and value change of the holding) &  NAC-S($\lambda$) algorithm & Data generated by a simulator & Proposes adversarial RL in market making\\
%   \hline
%   \citet{gavsperov2021market} &  Agent’s inventory; price range and trend predictions  & placing bid/ask orders with distances in tick size
% relative to the current best bid/ask  & symmetrically dampened PnL reward function in \cite{Spooner2018MM}, and inventory penalizing term & Policy gradient with fully-connected neural network & Bitstamp
% for the pair Bitcoin/US Dollar
% \\
  \hline
  
  \citet{Ganesh2019MM} & Trades executed in previous time step; Inventory; Reference 
mid-price and spread curves; Market share; & Pricing; Hedging;  & Total PnL with different penalty for inventory PnL & PPO & Data generated by their own simulator & Introduce a competing MM agent and let RL agent to learn its behavior\\ 
  \hline
\end{tabular}




\caption{RL Methods in Market Making}
\label{table:market_making}
\end{table}

\begin{table}[]
    \label{table:market_making_2}
    \caption{RL Methods in Market Making}
    \centering
\begin{tabular}{| m{2cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2cm} | m{2cm} |} 
  \hline
  Study & State & Action & Reward & Algorithm & Data & Contribution\\
  \hline
  \citet{mani2019applications} & volume imbalance and the market-maker’s bid-ask spread &changes in the
market-maker’s ask and bid quotes &a linear function of profit, inventory penalty 
and market-maker’s bid-ask spread & SARSA and Double SARSA & Using the simulator of their own & Use risk sensitive RL in market making
\\
  \hline
  \citet{spooner2020robust} & Current time and the agent's inventory &   Quoted spread and reservation price & Mark-to-market
(MtM) value of the agent's holding with penalty term of terminal inventory &  NAC-S($\lambda$) algorithm & Data generated by a simulator & Proposes adversarial RL in market making\\
  \hline
  \citet{gavsperov2021market} &  Agent’s inventory; price range and trend predictions  & placing bid/ask orders with distances in tick size
relative to the current best bid/ask  & symmetrically dampened PnL reward function in \cite{Spooner2018MM}, and inventory penalizing term & Policy optimization by genetic algorithms & Bitstamp
for the pair Bitcoin/US Dollar& Use  signal generating unit to predict price change
\\
\hline

\citet{selser2021optimal} & mid-price of the asset, inventory of the agent,  and time & (discretized) bid price and ask price &a profit minus the estimated variance of profit with a constant & Deep Q-Learning and Tabular Q-Learning & Using the simulator of their own & Use a mean minus variance formulation of reward to recover the optimal agent  
\\
\hline

\citet{haider2021gaussian} & volatility, relative strength index,
book imbalance, inventory, ask level and bid level & Place limit
orders at
fixed distances
to the mid-
price; Clear
inventory & a variant of asymmetrically dampened reward function proposed in \citet{Spooner2018MM} & Gaussian distribution based nonlinear
function approximation (GBNLFA, a variant of SARSA) & Data from their simulator, which is developed based on historical data & Propose the RL algorithm GBNLFA to handle function approximation from continuous states to discrete actions
\\
\hline


\end{tabular}
\end{table}


\begin{table}[H]
\caption{Surveyed paper for Reinforcement Learning in Portfolio Management}
\label{table:multi_stage_portfolio_management}
\begin{tabular}{| m{2cm} | m{3cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2.3cm} | }
\hline
Application & State& Action & Reward & Algorithm& Data \\ \hline
\cite{jiang2017deep} & Prices, Portfolio& Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency \\ \hline
\cite{yu2019model}& Prices, Portfolio, Market Indicators, Predictions & Asset Allocation Weight & Return& DDPG& Stock \\ \hline
\cite{zhang2020deep} & Prices, Portfolio, Technical Indicators& Long/Hold/Short & Volatility-Adjusted Return & PG, DQN, A2C & Futures \\ \hline
\cite{ye2020reinforcement} & Prices, Predictions & Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency, Stock \\ \hline
\cite{nan2020sentiment} & Prices, Portfolio, Predictions & Long/Hold/Short & Return& DQN & Stock \\ \hline
\cite{wang2021deeptrader} & Prices, Market Indicators, Predictions & Asset Allocation Weight & Return& Policy Gradient& Stock \\ \hline
\cite{wang2021commission} & Prices, Portfolio, LOB, Predictions & Asset Allocation Weight, Long/Hold/Short & Return& Reinforce, Double-Q & Stock \\ \hline
\cite{benhamou2020aamdrl} & Prices, Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio, Strategies \\ \hline
\cite{benhamou2021detecting} & Prices, Portfolio, Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio, Strategies \\ \hline
\end{tabular}
\end{table}


\input{Tables/table_optimal_execution}


==> Tables/tab_simulator_MM.tex <==
\begin{table}[]
    \centering
\begin{tabular}{m{2cm}  m{5 cm} m{7cm}} 
  \hline
  Literature & Security Mid-price Model & Investor Agent Model \\
  \hline

  \citet{chan2001electronic} & Poisson Jump Process &   Informed and uninformed trading
agent arrivals modeled by Poisson Process with constant intensity 
\\
  \hline
  \citet{mani2019applications} & Poisson Jump Process &   Informed and uninformed trading
agent arrivals modeled by Poisson Process with constant intensity
\\
  \hline

  \citet{selser2021optimal} & Brownian motion &   Investor agent orders modeled by Poisson processes with intensities being functions of the offset between the security price and the prices offered by the market maker \\
  \hline

  \citet{spooner2020robust} & Brownian motion with drift; drift parameter are not fixed but decided by adversary agent&   Investor agent orders modeled by Poisson processes with intensities being functions of the offset between the security price and the prices offered by the market maker; parameters of the function are not fixed but decided by adversary agent \\
  \hline

  \citet{Ganesh2019MM} & Geometric Brownian motion &   Investor agent orders are generated with a fixed probability at each timestep \\
  \hline


\end{tabular}
    \caption{Simulators of market making with RL}
    \label{table:market_making_simulators}
\end{table}




==> Tables/table_combined.tex <==

% NOTE : use \url{https://docs.google.com/spreadsheets/d/1s22i_gdk6T1hCaDyAsQdvsbaQGnyOFGzfSR2WUgPlpo/edit?usp=sharing} to update table 2


\begin{table}[H]
% \centering
\caption{Literature on RL methods: state and actions. }
\begin{tabular}{lp{0.1\textwidth}|llllllllll|llllll}
\hline
\multirow{2}{*}{}  & \multirow{2}{*}{Literature}  &  \multicolumn{10}{c|}{State} & \multicolumn{6}{c}{Action}\\ \cline{3-18} 
 &  & \rotatebox{90}{Price} & \rotatebox{90}{Inventory} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Company Info} & \rotatebox{90}{Predictions} & \rotatebox{90}{Bid-ask Info} & \rotatebox{90}{Trading Volume} & \rotatebox{90}{E2E} & \rotatebox{90}{Time} & \rotatebox{90}{Allocation Weight} & \rotatebox{90}{Long/Short} & \rotatebox{90}{Bid Price} & \rotatebox{90}{Quantity} & \rotatebox{90}{Place Limit Order} & \rotatebox{90}{Clear Inventory} \\ \hline
\multirow{20}{*}{\rotatebox{90}{Portfolio Management}} & \cite{jiang2017deep}  &  \cmark & \cmark  & & &  & & & & & & \cmark & & &  & &  \\
 &  \cite{yu2019model} &  \cmark & \cmark  & \cmark & &  & \cmark & & & & & \cmark & & &  & &  \\
 &  \cite{zhang2020deep}  &  \cmark & \cmark  & & \cmark  & & & & & & & & \cmark & &  & &  \\
 &  \cite{ye2020reinforcement}& \cmark & & & &  & & & & & & \cmark & & &  & &  \\
 &  \cite{wang2021deeptrader} & \cmark & & \cmark & &  & \cmark & & & & & \cmark & & &  & &  \\
 &  \cite{wang2021commission} & \cmark & \cmark  & & &  & \cmark & & \cmark & \cmark &  & \cmark & & &  & &  \\
 &  \cite{benhamou2021detecting} & \cmark & \cmark  & \cmark & &  & & & & & & \cmark & & &  & &  \\
 &  \cite{liu2018practical}  &  \cmark & \cmark  & & &  & & & & & & & \cmark & &  & &  \\
 &  \cite{wang2019alphastock} & \cmark & & & & \cmark  & & & \cmark & & & \cmark & & &  & &  \\
 &  \cite{li2019optimistic}  &  \cmark & \cmark  & & &  & & & & & & \cmark & & &  & &  \\
 &  \cite{park2020intelligent}& \cmark & \cmark  & & &  & & & & & & & \cmark & &  & &  \\
 &  \cite{gao2020application} & \cmark & \cmark  & & &  & & & & & & \cmark & & &  & &  \\
 &  \cite{koratamaddi2021market} & \cmark & \cmark  & & &  & \cmark & & & & & & \cmark & &  & &  \\
 &  \cite{yang2020deep}&  \cmark & \cmark  & & \cmark  & & & & & & & \cmark & & &  & &  \\
 &  \cite{liu2020adaptive}&  \cmark & \cmark  & & \cmark  & & & & & & & & \cmark & &  & &  \\
 &  \cite{theate2021application} & \cmark & \cmark  & & &  & & & & & & & \cmark & &  & &  \\
 &  \cite{lei2020time} &  \cmark & \cmark  & & &  & \cmark & & & & & & & &  & &  \\
 &  \cite{ma2021parallel} &  \cmark & \cmark  & & \cmark  & & & & & & & & \cmark & &  & &  \\
 &  \cite{lee2020maps} &  \cmark & & & &  & & & & & & & \cmark & &  & &  \\
 &  \cite{soleymani2021deep} &  \cmark & \cmark  & & \cmark  & & & & & & & \cmark & & &  & &  \\ \hline
\multirow{8}{*}{\rotatebox{90}{Optimal Execution}}  & \cite{nevmyvaka2006reinforcement} &  & \cmark  & & &  & & \cmark  &  \cmark & & \cmark  &  & & \cmark  &  & &  \\
 &  \cite{deng2016deep}  &  \cmark & & & &  & & & & & & & \cmark & &  & &  \\
 &  \cite{wei2019model}  & & \cmark  & & &  & & & & \cmark &  & & & & \cmark & &  \\
 &  \cite{lin2020E2E} & & \cmark  & & &  & & & & \cmark &  & & & & \cmark & &  \\
 &  \cite{fang2021universal} & \cmark & \cmark  & & &  & & & \cmark & & \cmark  &  & & & \cmark & &  \\
 &  \cite{lin2020deep}&  \cmark & \cmark  & & &  & & \cmark  &  & \cmark &  & & & & \cmark & &  \\
 &  \cite{shen2014risk}  & & \cmark  & & &  & & \cmark  &  & & & & & \cmark  &  & &  \\
 &  \cite{hendricks2014reinforcement} &  & \cmark  & & &  & & \cmark  &  \cmark & & \cmark  &  & & & \cmark & &  \\ \hline
\multirow{9}{*}{\rotatebox{90}{Market Making}}& \cite{chan2001electronic} & \cmark & \cmark  & & &  & & \cmark  &  & & & & & &  & \cmark &  \\
 &  \cite{Patel2018MM} &  \cmark & \cmark  & & &  & & & \cmark & \cmark &  \cmark  &  & & &  & \cmark &  \\
 &  \cite{Spooner2018MM}  &  \cmark & \cmark  & & \cmark  & & & \cmark  &  \cmark & & & & & &  & \cmark & \cmark  \\
 &  \cite{Ganesh2019MM}&  \cmark & \cmark  & & &  & & \cmark  &  \cmark & & & & & &  & \cmark &  \\
 &  \cite{mani2019applications}  &  & & & &  & & \cmark  &  & & & & & &  & \cmark &  \\
 &  \cite{spooner2020robust} & & \cmark  & & &  & & & & & \cmark  &  & & &  & \cmark &  \\
 &  \cite{gavsperov2021market}& \cmark & \cmark  & & &  & \cmark & & & & & & & &  & \cmark &  \\
 &  \cite{selser2021optimal} &  \cmark & \cmark  & & &  & & & & & \cmark  &  & & &  & \cmark &  \\
 &  \cite{haider2021gaussian} & \cmark & \cmark  & & \cmark  & & & \cmark  &  & & & & & &  & \cmark & \cmark  \\ \hline
\end{tabular}
\label{table:state_action}
\end{table}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[H]
\caption{Literature on RL methods: reward and algorithm. }
\label{table:reward+algo}
\begin{tabular}{lp{0.1\textwidth}|lllllll|lllllllllll}
\hline
\multirow{2}{*}{}                                      & \multirow{2}{*}{Literature}                  & \multicolumn{7}{l|}{Reward}                                                                                                                                                                 & \multicolumn{9}{l}{Algorithm}                                                                                                                                                                      &                              \\ \cline{3-20} 
                                                       &                                    & \rotatebox{90}{PnL} & \rotatebox{90}{Return} & \rotatebox{90}{VR} & \rotatebox{90}{IS} & \rotatebox{90}{Shaped reward} & \rotatebox{90}{Inventory Penalty} & \rotatebox{90}{Market Quality} & \rotatebox{90}{DQN} & \rotatebox{90}{PG} & \rotatebox{90}{DDPG} & \rotatebox{90}{A2C} & \rotatebox{90}{PPO} & \rotatebox{90}{simulator} & \rotatebox{90}{Q-learning} & \rotatebox{90}{SARSA} & \rotatebox{90}{NAC-S} & \rotatebox{90}{R-learning}& \rotatebox{90}{neuroevolution}\\ \hline
\multirow{20}{*}{\rotatebox{90}{Portfolio Management}} & \cite{jiang2017deep}               &                     & \cmark                 &                    &                    &                               &                                   &                                &                     & \cmark             &                      &                     &                     &                           &                             &                     &                              \\
                                                       & \cite{yu2019model}                 &                     & \cmark                 &                    &                    &                               &                                   &                                &                     &                    & \cmark               &                     &                     &                           &                             &                            &                       \\
                                                       & \cite{zhang2020deep}               &                     &                        & \cmark             &                    &                               &                                   &                                & \cmark              & \cmark             &                      & \cmark              &                     &                           &                       &                     &                       \\
                                                       & \cite{ye2020reinforcement}         &                     & \cmark                 &                    &                    &                               &                                   &                                &                     & \cmark             &                      &                     &                     &                           &                             &                    &                              \\
                                                       & \cite{wang2021deeptrader}          &                     & \cmark                 &                    &                    &                               &                                   &                                &                     & \cmark             &                      &                     &                     &                           &                             &                     &                              \\
                                                       & \cite{wang2021commission}          &                     & \cmark                 &                    &                    &                               &                                   &                                & \cmark              & \cmark             &                      &                     &                     &                           &                      &                    &                              \\
                                                       & \cite{benhamou2021detecting}       &                     & \cmark                 &                    &                    &                               &                                   &                                &                     & \cmark             &                      &                     &                     &                           &                             &                     &                              \\
                                                       & \cite{liu2018practical}            &                     & \cmark                 &                    &                    &                               &                                   &                                &                     &                    & \cmark               &                     &                     &                           &                             &                            &                       \\
                                                       & \cite{wang2019alphastock}          &                     &                        & \cmark             &                    &                               &                                   &                                &                     & \cmark             &                      &                     &                     &                           &                             &                     &                              \\
                                                       & \cite{li2019optimistic}            &                     & \cmark                 &                    &                    &                               &                                   &                                &                     &                    & \cmark               &                     &                     &                           &                             &                            &                        \\
                                                       & \cite{park2020intelligent}         &                     & \cmark                 &                    &                    &                               &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                      &                            &                              \\
                                                       & \cite{gao2020application}          &                     & \cmark                 &                    &                    &                               &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                      &                            &                              \\
                                                       & \cite{koratamaddi2021market}       &                     &                        &                    &                    & \cmark                        &                                   &                                &                     &                    & \cmark               &                     &                     &                           &                             &                            &                       \\
                                                       & \cite{yang2020deep}                &                     &                        &                    &                    & \cmark                        &                                   &                                &                     &                    & \cmark               & \cmark              & \cmark              &                           &                             &                     &                        \\
                                                       & \cite{liu2020adaptive}             &                     &                        & \cmark             &                    &                               &                                   &                                &                     & \cmark             &                      &                     &                     &                           &                             &                     &                              \\
                                                       & \cite{theate2021application}       &                     & \cmark                 &                    &                    &                               &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                       &                            &                              \\
                                                       & \cite{lei2020time}                 &                     & \cmark                 &                    &                    &                               &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                      &                            &                              \\
                                                       & \cite{ma2021parallel}              &                     & \cmark                 &                    &                    &                               &                                   &                                &                     & \cmark             &                      &                     &                     &                           &                      &                            &                              \\
                                                       & \cite{lee2020maps}                 &                     &                        &                    &                    & \cmark                        &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                      &                            &                              \\
                                                       & \cite{soleymani2021deep}           &                     &                        &                    & \cmark             &                               &                                   &                                &                     &                    &                      & \cmark              &                     &                           &                             &                            &                       \\ \hline
\multirow{8}{*}{\rotatebox{90}{Optimal Execution}}     & \cite{nevmyvaka2006reinforcement} & \cmark              &                        &                    &                    &                               &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                             &                            &                              \\
                                                       & \cite{deng2016deep}               & \cmark              &                        & \cmark             &                    &                               &                                   &                                &                     & \cmark             &                      &                     &                     &                           &                             &                            &                              \\
                                                       & \cite{wei2019model}               & \cmark              &                        &                    &                    &                               &                                   &                                &                     &                    &                      &                     &                     & \cmark                    &                             &                            &                              \\
                                                       & \cite{lin2020E2E}                 &                     &                        &                    & \cmark             &                               &                                   &                                &                     &                    &                      &                     & \cmark              &                           &                             &                            &                              \\
                                                       & \cite{fang2021universal}          &                     &                        &                    &                    & \cmark                        &                                   &                                &                     &                    &                      &                     & \cmark              &                           &                             &                            &                              \\
                                                       & \cite{lin2020deep}                &                     &                        &                    &                    & \cmark                        &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                             &                            &                              \\
                                                       & \cite{shen2014risk}               & \cmark              &                        &                    &                    &                               &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                             &                            &                              \\
                                                       & \cite{hendricks2014reinforcement} &                     &                        &                    & \cmark             &                               &                                   &                                & \cmark              &                    &                      &                     &                     &                           &                             &                            &                              \\ \hline
\multirow{9}{*}{\rotatebox{90}{Market Making}}         & \cite{chan2001electronic}          & \cmark              &                        &                    &                    &                               & \cmark                            & \cmark                         &                     &                    &                      &                     &                     &                           &                      &   \cmark                          &     &                    \\
                                                       & \cite{Patel2018MM}                 & \cmark              &                        &                    &                    &                               &                                   &                                &                     \cmark  &                    &                      &                     &                     &                           &                      &                            &                             &  \\
                                                       & \cite{Spooner2018MM}               & \cmark              &                        &                    &                    &                               & \cmark                            &                                &                     &                    &                      &                     &                     &                           & \cmark                      &   \cmark                           &    &  \cmark                            \\
                                                       & \cite{Ganesh2019MM}                & \cmark              &                        &                    &                    &                               & \cmark                            &                                &                     &                    &                      &                     &                    \cmark &                           &                             &                      &                              \\
                                                       & \cite{mani2019applications}        & \cmark              &                        &                    &                    &                               & \cmark                            & \cmark                         &                     &                    &                      &                     &                     &                           &                       &     \cmark                       &  &                             \\
                                                       & \cite{spooner2020robust}           & \cmark              &                        &                    &                    &                               & \cmark                            &                                &                     &                    &                      &                     &                     &                           &                             &                      &     \cmark                          & \\
                                                       & \cite{gavsperov2021market}         & \cmark              &                        &                    &                    &                               & \cmark                            &                                &                     &                    &                      &                     &                     &                           &                             &                      &                              & &\cmark \\
                                                       & \cite{selser2021optimal}           & \cmark              &                        &                    &                    &                               &                                   &                                &                     &                    &                      &                     &                     &                           & \cmark                      &                            &                              &  \\
                                                       & \cite{haider2021gaussian}          & \cmark              &                        &                    &                    &                               & \cmark                            &                                &                     &                    &                      &                     &                     &                           &                     &        \cmark                      &                               & \\ \hline
\end{tabular}
\label{table:reward_algo}
\end{table}


%  \begin{table}[]
% \caption{Literature on RL methods: reward and algorithm. 
% }
% \label{table:TODO}
% \begin{tabular}{c|c|ccccccc|cccccc}
% \cline{1-15} 
% \multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{Reward} & \multicolumn{4}{c}{Algorithm} \\ \cline{3-15} 
%  & & \rotatebox{90}{PnL} & \rotatebox{90}{Return} & \rotatebox{90}{VR} & \rotatebox{90}{IS} & \rotatebox{90}{Shaped reward} & \rotatebox{90}{Inventory Penalty} & \rotatebox{90}{Market Quality} & \rotatebox{90}{DQN} & \rotatebox{90}{PG} & \rotatebox{90}{PPO} & \rotatebox{90}{simulator} & \rotatebox{90}{TBD} & \rotatebox{90}{TBD} \\ \hline
% \multirow{9}{*}{\rotatebox{90}{Portfolio Management}} 
% & \cite{jiang2017deep} & & \cmark & & & & & & & & & \red{TBD} & & \\
%  & \cite{yu2019model} & & \cmark & & & & & & & & & & & \\
%  & \cite{zhang2020deep} & & \cmark & & & & & & & & & & & \\
%  &\cite{ye2020reinforcement} & & & \cmark & & & & & & & & & & \\
%  &\cite{nan2020sentiment} & & \cmark & & & & & & & & & & & \\
%  &\cite{wang2021deeptrader} & & \cmark & & & & & & & & & & & \\
%  & \cite{wang2021commission} & & \cmark & & & & & & & & & & & \\
%  & \cite{benhamou2020aamdrl} & & \cmark & & & & & & & & & & & \\
% & \cite{benhamou2021detecting} & & \cmark & & & & & & & & & & & \\ \cline{1-15} 
% \multirow{8}{*}{\rotatebox{90}{Optimal Execution}} & 
% \citet{nevmyvaka2006reinforcement} & \cmark & & & & & & & \cmark & & & & & \\
%  & \citet{deng2016deep} & \cmark & & \cmark & & & & & & \cmark & & & & \\
%  & \citet{wei2019model} &\cmark & & & & & & & & & & \cmark & & \\
%  & \citet{lin2020E2E} & & & & \cmark & & & & & & \cmark & & & \\
%  & \citet{fang2021universal} & & & & &\cmark & & & & & \cmark & & & \\
% & \citet{lin2020deep} & & & & &\cmark & & & \cmark & & & & & \\
%  & \citet{shen2014risk} & \cmark & & & & & & & \cmark & & & & & \\
%  &\citet{hendricks2014reinforcement} & & & &\cmark & & & & \cmark & & & & & 
%  \\\cline{1-15} 
% \end{tabular}
% \end{table}


%  \begin{table}[]
% \caption{Literature on RL methods in Market Making: reward and algorithm. 
% }
% \label{table:TODO}
% \begin{tabular}{c|c|ccccccc|cccccc}
% \cline{1-15} 
% \multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{Reward} & \multicolumn{4}{c}{Algorithm} \\ \cline{3-15} 
%  & & \rotatebox{90}{PnL} & \rotatebox{90}{Return} & \rotatebox{90}{VR} & \rotatebox{90}{IS} & \rotatebox{90}{Shaped reward} & \rotatebox{90}{Inventory Penalty} & \rotatebox{90}{Market Quality} & \rotatebox{90}{Critic-only} & \rotatebox{90}{Actor-only} & \rotatebox{90}{Actor-critic} \\ \hline
% \multirow{9}{*}{\rotatebox{90}{Market Making}} 
% & \cite{chan2001electronic} &\cmark &  & & & &\cmark &\cmark &\cmark & & \cmark \\
% & \cite{Patel2018MM} &\cmark &  & & & & & &\cmark & &  \\
% & \cite{Spooner2018MM} &\cmark &  & & & &\cmark & &\cmark & &  \\
% & \cite{Ganesh2019MM} &\cmark &  & & & &\cmark & & &\cmark &  \\
% & \cite{mani2019applications} &\cmark &  & & & &\cmark & \cmark &\cmark & &  \\
% & \cite{spooner2020robust} &\cmark &  & & & &\cmark & & &\cmark &  \\
% & \cite{gavsperov2021market} &\cmark &  & & & &\cmark & & &\cmark &  \\
% & \cite{selser2021optimal} &\cmark &  & & & & & &\cmark & &  \\
% & \cite{haider2021gaussian} &\cmark &  & & & &\cmark  & &\cmark & &  \\

% \cline{1-15} 

% \end{tabular}
% \end{table}


% \begin{table}[]
% %\resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllll@{}}
% \hline
% Paper & MDP & Algorithm & Data & Contribution \\
% \hline
%\citet{jiang2017deep} & 
%\begin{tabular}[c]{@{}l@{}}State: Stock price and asset weight at prior time\\ Action:\\ Reward\end{tabular} & 
%\acrshort{DPG}& 
%11 top volume cryptocurrencies & 
%Proposed "Ensemble of Identical Independent Evaluators""; Applied a stochastic mini-batch online learning scheme\\
% \hline
%\citet{ye2020reinforcement} & \begin{tabular}[c]{@{}l@{}}State\\ Action\\ Reward\end{tabular} & & & \\
% \hline
%\citet{nan2020sentiment} & & & & \\
% \hline
%\citet{liang2018adversarial} & & & & \\
% \hline
%\citet{liu2020adaptive} & & & & \\
% \hline
%\citet{zhang2020deep} & & & & \\
% \hline
%\citet{wang2021commission} & & & & \\
% \hline 
%\citet{wang2021deeptrader} & & & & \\
% \hline
% \end{tabular}
% %%
% %}
% \label{table:multi_stage_portfolio_management}
% \caption{PM}
% \end{table}


% \begin{table}[H]
% \begin{tabular}{| m{2cm} | m{2.5cm}| m{2.5cm} | m{2cm} |m{1.7cm} |m{2.5cm} | m{2cm} |}
% \hline
% Application & State & Action & Reward & Algorithm& Data & Contribution \\ \hline
% \cite{jiang2017deep} & Asset Info Portfolio Info & Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency & \\ \hline
% \cite{yu2019model}& Asset Info Portfolio Info, Market Indicators, Other & Asset Allocation Weight & Return& DDPG& Stock & \\ \hline
% \cite{zhang2020deep} & Asset Info Portfolio Info, Technical Indicators& Long/Short Proportion & Volatility-Adjusted Return & PG, DQN, A2C & Futures & \\ \hline
% \cite{ye2020reinforcement} & Asset Info Other & Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency, Stock & \\ \hline
% \cite{nan2020sentiment} & Asset Info, Portfolio Info, Other & Long/Hold/Short Proportion & Return& DQN & Stock & \\ \hline
% \cite{wang2021deeptrader} & Asset Info, Market Indicators, Other& Asset Allocation Weight & Return& Policy Gradient& Stock & \\ \hline
% \cite{wang2021commission} & Asset Info, Portfolio Info, LOB, Other & Asset Allocation Weight, Long/Hold/Short & Return& Reinforce, Double-Q & Stock & \\ \hline
% \cite{benhamou2020aamdrl} & Asset Info Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio/Strategies & \\ \hline
% \cite{benhamou2021detecting} & Asset InfoPortfolio Info, Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio/Strategies & \\ \hline
% \end{tabular}
% \label{table:multi_stage_portfolio_management}
% \caption{Surveyed paper for Reinforcement Learning in Portfolio Management}
% \end{table}


% \begin{table}[]
% % \begin{tabular}{mmmmmm}
% \begin{tabular}{| m{2cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2cm} | }
% \hline
% Application & State & Action & Reward & Algorithm & Data \\ \hline
% A deep reinforcement learning framework for the financial portfolio management problem & Price (low, high, close) normalized by the latest closing price; Internal state is the weight at t-1. & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DPG& Top 11 volume bitcoin trading information from Poloniex \\ \hline
% Reinforcement-Learning-based Portfolio Management with Augmented Asset Movement Prediction States & Price (low, high, close); Articles from the news. & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DPG; PPO; PG & Bitcoin data; stock from HighTech companies\\ \hline
% Adversarial Deep Reinforcement Learning in Portfolio Management & Price (low, high, close); Volume; Other financial indexes.& Weights vector to determine portfolio allocation. & Cumulative return subtract portfolio volatility & DDPG; PPO; PG& Use data from a simulator which is developed based on historical data \\ \hline
% %%
% Model-based deep reinforcement learning for dynamic portfolio optimization & Price (low, high, close); Augmented states (predicted future price change percentage) & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DDPG & Company stocks\\ \hline
% %%
% Adaptive Quantitative Trading An Imitative Deep Reinforcement Learning Approach & Account observation set, Market observation set& Long or short & Sharpe ratio differential & Imitative Recurrent DPG & CHINA IC, IF \\ \hline
% %%
% \end{tabular}
% \caption{PM}
% \end{table}

% \multirow{9}{*}{\rotatebox{0}{\makecell{Portfolio \\ Management}}}

% \begin{table}[]
% \begin{tabular}{l|l|lllllllll|llll}
% \multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{l|}{State} & \multicolumn{4}{l}{Action} \\ \cline{3-15} 
% & & \rotatebox{90}{Price} & \rotatebox{90}{Inventory/Portfolio} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Predictions} & \rotatebox{90}{Spread} & \rotatebox{90}{Volume} & \rotatebox{90}{E2E/LOB} & \rotatebox{90}{Time} & \rotatebox{90}{Allocation Weight} & \rotatebox{90}{Long/Short} & \rotatebox{90}{Bid Price} & \rotatebox{90}{Quantity} \\ \hline
% \cite{jiang2017deep} & \multirow{9}{*}{\rotatebox{90}{Portfolio Management}} & \cmark & \cmark & & & & & & & & \cmark & & & \\
% \cite{yu2019model} & & \cmark & \cmark & \cmark & & \cmark & & & & & \cmark & & & \\
% \cite{zhang2020deep} & & \cmark & \cmark & & \cmark & & & & & & & \cmark & & \\
% \cite{ye2020reinforcement} & & \cmark & & & & & & & & & \cmark & & & \\
% \cite{nan2020sentiment} & & \cmark & \cmark & & & & & & & & & \cmark & & \\
% \cite{wang2021deeptrader}& & \cmark & & \cmark & & \cmark & & & & & \cmark & & & \\
% \cite{wang2021commission}& & \cmark & \cmark & & & \cmark & & & \cmark & & \cmark & & & \\
% \cite{benhamou2020aamdrl}& & \cmark & & \cmark & & & & & & & \cmark & & & \\
% \cite{benhamou2021detecting} & & \cmark & \cmark & \cmark & & & & & & & \cmark & & & \\ \cline{2-15} 
% \citet{nevmyvaka2006reinforcement} & 
% \multirow{8}{*}{\rotatebox{90}{Optimal Execution}} & & \cmark & & & & \cmark & \cmark & & \cmark & & & \cmark & \\
% \citet{deng2016deep} & & \cmark & & & & & & & & & & \cmark & & \\
% \citet{wei2019model} & & & \cmark & & & & & & \cmark & & & & & \cmark \\
% \citet{lin2020E2E} & & & \cmark & & & & & & \cmark & & & & & \cmark \\
% \citet{fang2021universal}& & \cmark & \cmark & & & & & \cmark & & \cmark & & & & \cmark \\
% \citet{lin2020deep}& & \cmark & \cmark & & & & \cmark & & \cmark & & & & & \cmark \\
% \citet{shen2014risk} & & & \cmark & & & & \cmark & & & & & & \cmark & \\
% \citet{hendricks2014reinforcement} & & & \cmark & & & & \cmark & \cmark & & \cmark & & & & \cmark 
% \end{tabular}
% \end{table}


% Portfolio
% E2E

% \begin{table}[]
% \centering
% \caption{Literature on RL methods: state and actions. 
% }
% \label{table:TODO}
% \begin{tabular}{c|c|ccccccccc|cccccc}
% \cline{1-17} 
% \multirow{2}{*}{Area} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{State} & \multicolumn{6}{c}{Action} \\ \cline{3-17} 
%  & & \rotatebox{90}{Price} & \rotatebox{90}{Inventory} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Predictions} & \rotatebox{90}{Bid-ask information} & \rotatebox{90}{Trading Volume} & \rotatebox{90}{E2E} & \rotatebox{90}{Time} & \rotatebox{90}{Allocation Weight} & \rotatebox{90}{Long/Short} & \rotatebox{90}{Bid Price} & \rotatebox{90}{Quantity} & \rotatebox{90}{Place Limit Order} & \rotatebox{90}{Clear Inventory} \\ \hline
% \multirow{9}{*}{\rotatebox{90}{Portfolio Management}} 

% & \cite{jiang2017deep} & \cmark & \cmark & & & & & & & & \cmark & & & \\

%  & \cite{yu2019model} & \cmark & \cmark & \cmark & & \cmark & & & & & \cmark & & & \\
 
%  & \cite{zhang2020deep} & \cmark & \cmark & & \cmark & & & & & & & \cmark & & \\
 
%  &\cite{ye2020reinforcement} & \cmark & & & & & & & & & \cmark & & & \\
 
%  &\cite{nan2020sentiment}& \cmark & \cmark & & & & & & & & & \cmark & & \\
 
%  &\cite{wang2021deeptrader} & \cmark & & \cmark & & \cmark & & & & & \cmark & & & \\
 
%  & \cite{wang2021commission} & \cmark & \cmark & & & \cmark & & & \cmark & & \cmark & & & \\
 
%  & \cite{benhamou2020aamdrl} & \cmark & & \cmark & & & & & & & \cmark & & & \\
% &
% \cite{benhamou2021detecting} & \cmark & \cmark & \cmark & & & & & & & \cmark & & & \\ \cline{1-17} 


% \multirow{8}{*}{\rotatebox{90}{Optimal Execution}} 
% & 
% \citet{nevmyvaka2006reinforcement} & & \cmark & & & & \cmark & \cmark & & \cmark & & & \cmark & \\

%  & \citet{deng2016deep} & \cmark & & & & & & & & & & \cmark & & \\

%  & \citet{wei2019model} & & \cmark & & & & & & \cmark & & & & & \cmark \\
 
%  & \citet{lin2020E2E} & & \cmark & & & & & & \cmark & & & & & \cmark \\
 
%  & \citet{fang2021universal} & \cmark & \cmark & & & & & \cmark & & \cmark & & & & \cmark \\

% & \citet{lin2020deep} & \cmark & \cmark & & & & \cmark & & \cmark & & & & & \cmark \\

%  & \citet{shen2014risk} & & \cmark & & & & \cmark & & & & & & \cmark & \\
 
%  &\citet{hendricks2014reinforcement} & & \cmark & & & & \cmark & \cmark & & \cmark & & & & \cmark \\
%  \cline{1-17} 
%  \multirow{9}{*}{\rotatebox{90}{Market Making}}
%  & \cite{chan2001electronic} & \cmark & \cmark  & & & & \cmark  & & & & & & & & \cmark &  \\

% & \cite{Patel2018MM} & \cmark & \cmark & & & & &  \cmark  &  \cmark  & \cmark & & & & & \cmark & \\


% & \cite{Spooner2018MM} & \cmark & \cmark  & &\cmark  & &  \cmark &  \cmark  & & & & & & & \cmark & \cmark  \\

% & \cite{Ganesh2019MM} & \cmark & \cmark  & &  & &  \cmark &  \cmark  & & & & & & &  \cmark & \\

% & \cite{mani2019applications} &  & & &  & &  \cmark & & &  & & & & & \cmark &  \\

% & \cite{spooner2020robust} &  &  \cmark  & &  & & & & &\cmark & & & &  & \cmark &\\

% & \cite{gavsperov2021market} &\cmark &\cmark  & &  & \cmark & & & &  & & & & & \cmark &  \\

% & \cite{selser2021optimal} &\cmark &\cmark  & &  & & & & &\cmark  &  & & &  & \cmark &  \\

% & \cite{haider2021gaussian} & \cmark &  \cmark  & &  \cmark  &  &\cmark & & & & & & &  & \cmark &  \cmark\\
%\cline{1-17} 
% \end{tabular}
% \end{table}


==> Tables/table_market_making.tex <==


\begin{table}[]
\caption{Literature on RL methods in market making: state and actions.
}
\label{newtable:market_making_2}
\begin{tabular}{c|c|ccccccccc|cccc}
\cline{1-15} 
\multirow{2}{*}{Study}             & \multirow{2}{*}{Application}                                     & \multicolumn{9}{c|}{State}                                                                                                                                                                                                                                            & \multicolumn{2}{c}{Action}                                                                                            \\ \cline{3-15} 
                                   &                                                       & \rotatebox{90}{Price} & \rotatebox{90}{Inventory/Portfolio} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Predictions} & \rotatebox{90}{Bid-ask information} & \rotatebox{90}{Trading Volume} & \rotatebox{90}{E2E} & \rotatebox{90}{Time} & \rotatebox{90}{Place limit order} & \rotatebox{90}{Clear Inventory} \\ \hline
% \multirow{9}{*}{\rotatebox{90}{MM}}

& \cite{chan2001electronic}    & \cmark                & \cmark                              &                                  &                                     &                             & \cmark                       &                      &                         &                      & \cmark                            &                            &                           &                          \\

& \cite{Patel2018MM}    & \cmark                & \cmark                             &                                  &                                     &                             &                        &  \cmark                       &  \cmark                       & \cmark                     & \cmark                            &                            &                           &                          \\


& \cite{Spooner2018MM}    & \cmark                & \cmark                              &                                  &   \cmark                                   &                             &  \cmark                        &     \cmark                    &                         &                      & \cmark                            & \cmark                            &                           &                          \\

& \cite{Ganesh2019MM}    & \cmark                & \cmark                              &                                  &                                    &                             &  \cmark                        &     \cmark                    &                         &                      & \cmark                            &                            &                           &                          \\

& \cite{mani2019applications}    &              &                            &                                  &                                    &                             &  \cmark                        &                        &                         &                      & \cmark                            &                            &                           &                          \\

& \cite{spooner2020robust}    &              &  \cmark                          &                                  &                                    &                             &                      &                      &                         &   \cmark                   & \cmark                            &                            &                           &                          \\

& \cite{gavsperov2021market}    &   \cmark              &  \cmark                          &                                  &                                    &    \cmark                            &                      &                      &                         &                 & \cmark                            &                            &                           &                          \\

& \cite{selser2021optimal}    &   \cmark              &  \cmark                          &                                  &                                    &                                &                      &                      &                         &   \cmark              & \cmark                            &                            &                           &                          \\

& \cite{haider2021gaussian}    & \cmark                &  \cmark                          &                                  &     \cmark                                 &                                &   \cmark                      &                        &                         &                 & \cmark                            &  \cmark                           &                           &                          \\

          \cline{1-15} 
\end{tabular}
\end{table}


 \begin{table}[]
\caption{Literature on RL methods in Market Making: reward and algorithm. 
}
\label{table:TODO}
\begin{tabular}{c|c|ccccccc|cccccc}
\cline{1-15} 
\multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{Reward} & \multicolumn{4}{c}{Algorithm} \\ \cline{3-15} 
 & & \rotatebox{90}{PnL} & \rotatebox{90}{Return} & \rotatebox{90}{VR} & \rotatebox{90}{IS} & \rotatebox{90}{Shaped reward} & \rotatebox{90}{Inventory Penalty} & \rotatebox{90}{Market Quality} & \rotatebox{90}{Critic-only} & \rotatebox{90}{Actor-only} & \rotatebox{90}{Actor-critic} \\ \hline
\multirow{9}{*}{\rotatebox{90}{Market Making}} 
& \cite{chan2001electronic} &\cmark &  & & & &\cmark &\cmark      &\cmark & & \cmark \\
& \cite{Patel2018MM} &\cmark &  & & & & &          &\cmark & &  \\
& \cite{Spooner2018MM} &\cmark &  & & & &\cmark &          &\cmark & &  \\
& \cite{Ganesh2019MM} &\cmark &  & & & &\cmark &          & &\cmark &  \\
& \cite{mani2019applications} &\cmark &  & & & &\cmark & \cmark         &\cmark & &  \\
& \cite{spooner2020robust} &\cmark &  & & & &\cmark &         & &\cmark &  \\
& \cite{gavsperov2021market} &\cmark &  & & & &\cmark &         & &\cmark &  \\
& \cite{selser2021optimal} &\cmark &  & & & & &         &\cmark & &  \\
& \cite{haider2021gaussian} &\cmark &  & & & &\cmark  &         &\cmark & &  \\

\cline{1-15} 

\end{tabular}
\end{table}

==> Tables/table_multi_stage_portfolio_management.tex <==
% \begin{table}[]
% %\resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}lllll@{}}
% \hline
% Paper & MDP & Algorithm & Data & Contribution \\
% \hline
%\citet{jiang2017deep} & 
%\begin{tabular}[c]{@{}l@{}}State: Stock price and asset weight at prior time\\ Action:\\ Reward\end{tabular} & 
%\acrshort{DPG}& 
%11 top volume cryptocurrencies & 
%Proposed "Ensemble of Identical Independent Evaluators""; Applied a stochastic mini-batch online learning scheme\\
% \hline
%\citet{ye2020reinforcement} & \begin{tabular}[c]{@{}l@{}}State\\ Action\\ Reward\end{tabular} & & & \\
% \hline
%\citet{nan2020sentiment} & & & & \\
% \hline
%\citet{liang2018adversarial} & & & & \\
% \hline
%\citet{liu2020adaptive} & & & & \\
% \hline
%\citet{zhang2020deep} & & & & \\
% \hline
%\citet{wang2021commission} & & & & \\
% \hline 
%\citet{wang2021deeptrader} & & & & \\
% \hline
% \end{tabular}
% %%
% %}
% \label{table:multi_stage_portfolio_management}
% \caption{PM}
% \end{table}


% \begin{table}[H]
% \begin{tabular}{| m{2cm} | m{2.5cm}| m{2.5cm} | m{2cm} |m{1.7cm} |m{2.5cm} | m{2cm} |}
% \hline
% Application & State & Action & Reward & Algorithm& Data & Contribution \\ \hline
% \cite{jiang2017deep} & Asset Info Portfolio Info & Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency & \\ \hline
% \cite{yu2019model}& Asset Info Portfolio Info, Market Indicators, Other & Asset Allocation Weight & Return& DDPG& Stock & \\ \hline
% \cite{zhang2020deep} & Asset Info Portfolio Info, Technical Indicators& Long/Short Proportion & Volatility-Adjusted Return & PG, DQN, A2C & Futures & \\ \hline
% \cite{ye2020reinforcement} & Asset Info Other & Asset Allocation Weight & Return& Policy Gradient& Cryptocurrency, Stock & \\ \hline
% \cite{nan2020sentiment} & Asset Info, Portfolio Info, Other & Long/Hold/Short Proportion & Return& DQN & Stock & \\ \hline
% \cite{wang2021deeptrader} & Asset Info, Market Indicators, Other& Asset Allocation Weight & Return& Policy Gradient& Stock & \\ \hline
% \cite{wang2021commission} & Asset Info, Portfolio Info, LOB, Other & Asset Allocation Weight, Long/Hold/Short & Return& Reinforce, Double-Q & Stock & \\ \hline
% \cite{benhamou2020aamdrl} & Asset Info Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio/Strategies & \\ \hline
% \cite{benhamou2021detecting} & Asset InfoPortfolio Info, Market Indicators & Asset Allocation Weight & Return& Policy Gradient& Portfolio/Strategies & \\ \hline
% \end{tabular}
% \label{table:multi_stage_portfolio_management}
% \caption{Surveyed paper for Reinforcement Learning in Portfolio Management}
% \end{table}


% \begin{table}[]
% % \begin{tabular}{mmmmmm}
% \begin{tabular}{| m{2cm} | m{2.5cm}| m{2.5cm} | m{2.5cm} |m{1.7cm} |m{2cm} | }
% \hline
% Application & State & Action & Reward & Algorithm & Data \\ \hline
% A deep reinforcement learning framework for the financial portfolio management problem & Price (low, high, close) normalized by the latest closing price; Internal state is the weight at t-1. & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DPG& Top 11 volume bitcoin trading information from Poloniex \\ \hline
% Reinforcement-Learning-based Portfolio Management with Augmented Asset Movement Prediction States & Price (low, high, close); Articles from the news. & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DPG; PPO; PG & Bitcoin data; stock from HighTech companies\\ \hline
% Adversarial Deep Reinforcement Learning in Portfolio Management & Price (low, high, close); Volume; Other financial indexes.& Weights vector to determine portfolio allocation. & Cumulative return subtract portfolio volatility & DDPG; PPO; PG& Use data from a simulator which is developed based on historical data \\ \hline
% %%
% Model-based deep reinforcement learning for dynamic portfolio optimization & Price (low, high, close); Augmented states (predicted future price change percentage) & Weights vector to determine portfolio allocation. & Final portfolio value, i.e. average logarithmic cumulated return. & DDPG & Company stocks\\ \hline
% %%
% Adaptive Quantitative Trading An Imitative Deep Reinforcement Learning Approach & Account observation set, Market observation set& Long or short & Sharpe ratio differential & Imitative Recurrent DPG & CHINA IC, IF \\ \hline
% %%
% \end{tabular}
% \caption{PM}
% \end{table}

% \multirow{9}{*}{\rotatebox{0}{\makecell{Portfolio \\ Management}}}

% \begin{table}[]
% \begin{tabular}{l|l|lllllllll|llll}
% \multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{l|}{State} & \multicolumn{4}{l}{Action} \\ \cline{3-15} 
% & & \rotatebox{90}{Price} & \rotatebox{90}{Inventory/Portfolio} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Predictions} & \rotatebox{90}{Spread} & \rotatebox{90}{Volume} & \rotatebox{90}{E2E/LOB} & \rotatebox{90}{Time} & \rotatebox{90}{Allocation Weight} & \rotatebox{90}{Long/Short} & \rotatebox{90}{Bid Price} & \rotatebox{90}{Quantity} \\ \hline
% \cite{jiang2017deep} & \multirow{9}{*}{\rotatebox{90}{Portfolio Management}} & \cmark& \cmark & & & & & & & & \cmark & & & \\
% \cite{yu2019model} & & \cmark& \cmark & \cmark& & \cmark& & & & & \cmark & & & \\
% \cite{zhang2020deep} & & \cmark& \cmark & & \cmark & & & & & & & \cmark & & \\
% \cite{ye2020reinforcement} & & \cmark& & & & & & & & & \cmark & & & \\
% \cite{nan2020sentiment} & & \cmark& \cmark & & & & & & & & & \cmark & & \\
% \cite{wang2021deeptrader}& & \cmark& & \cmark& & \cmark& & & & & \cmark & & & \\
% \cite{wang2021commission}& & \cmark& \cmark & & & \cmark& & & \cmark & & \cmark & & & \\
% \cite{benhamou2020aamdrl}& & \cmark& & \cmark& & & & & & & \cmark & & & \\
% \cite{benhamou2021detecting} & & \cmark& \cmark & \cmark& & & & & & & \cmark & & & \\ \cline{2-15} 
% \citet{nevmyvaka2006reinforcement} & 
% \multirow{8}{*}{\rotatebox{90}{Optimal Execution}} & & \cmark & & & & \cmark & \cmark & & \cmark & & & \cmark & \\
% \citet{deng2016deep} & & \cmark& & & & & & & & & & \cmark & & \\
% \citet{wei2019model} & & & \cmark & & & & & & \cmark & & & & & \cmark \\
% \citet{lin2020E2E} & & & \cmark & & & & & & \cmark & & & & & \cmark \\
% \citet{fang2021universal}& & \cmark& \cmark & & & & & \cmark & & \cmark & & & & \cmark \\
% \citet{lin2020deep}& & \cmark& \cmark & & & & \cmark & & \cmark & & & & & \cmark \\
% \citet{shen2014risk} & & & \cmark & & & & \cmark & & & & & & \cmark & \\
% \citet{hendricks2014reinforcement} & & & \cmark & & & & \cmark & \cmark & & \cmark & & & & \cmark 
% \end{tabular}
% \end{table}


% Portfolio
% E2E

\begin{table}[]
\caption{Literature on RL methods: state and actions. 
}
\label{table:TODO}
\begin{tabular}{c|c|ccccccccc|cccc}
\cline{1-15} 
\multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{State} & \multicolumn{4}{c}{Action} \\ \cline{3-15} 
 & & \rotatebox{90}{Price} & \rotatebox{90}{Inventory} & \rotatebox{90}{Market Indicator} & \rotatebox{90}{Technical Indicator} & \rotatebox{90}{Predictions} & \rotatebox{90}{Bid-ask information} & \rotatebox{90}{Trading Volume} & \rotatebox{90}{E2E} & \rotatebox{90}{Time} & \rotatebox{90}{Allocation Weight} & \rotatebox{90}{Long/Short} & \rotatebox{90}{Bid Price} & \rotatebox{90}{Quantity} \\ \hline
\multirow{9}{*}{\rotatebox{90}{Portfolio Management}} & \cite{jiang2017deep} & \cmark& \cmark & & & & & & & & \cmark & & & \\
 & \cite{yu2019model} & \cmark& \cmark & \cmark& & \cmark& & & & & \cmark & & & \\
 & \cite{zhang2020deep} & \cmark& \cmark & & \cmark & & & & & & & \cmark & & \\
 &\cite{ye2020reinforcement} & \cmark& & & & & & & & & \cmark & & & \\
 &\cite{nan2020sentiment}& \cmark& \cmark & & & & & & & & & \cmark & & \\
 &\cite{wang2021deeptrader} & \cmark& & \cmark& & \cmark& & & & & \cmark & & & \\
 & \cite{wang2021commission} & \cmark& \cmark & & & \cmark& & & \cmark & & \cmark & & & \\
 & \cite{benhamou2020aamdrl} & \cmark& & \cmark& & & & & & & \cmark & & & \\
& \cite{benhamou2021detecting} & \cmark& \cmark & \cmark& & & & & & & \cmark & & & \\ \cline{1-15} 
\multirow{8}{*}{\rotatebox{90}{Optimal Execution}} & 
\citet{nevmyvaka2006reinforcement} & & \cmark & & & & \cmark & \cmark & & \cmark & & & \cmark & \\
 & \citet{deng2016deep} & \cmark& & & & & & & & & & \cmark & & \\
 & \citet{wei2019model} & & \cmark & & & & & & \cmark & & & & & \cmark \\
 & \citet{lin2020E2E} & & \cmark & & & & & & \cmark & & & & & \cmark \\
 & \citet{fang2021universal} & \cmark& \cmark & & & & & \cmark & & \cmark & & & & \cmark \\
& \citet{lin2020deep} & \cmark& \cmark & & & & \cmark & & \cmark & & & & & \cmark \\
 & \citet{shen2014risk} & & \cmark & & & & \cmark & & & & & & \cmark & \\
 &\citet{hendricks2014reinforcement} & & \cmark & & & & \cmark & \cmark & & \cmark & & & & \cmark \\\cline{1-15} 
\end{tabular}
\end{table}



 \begin{table}[]
\caption{Literature on RL methods: reward and algorithm. 
}
\label{table:TODO}
\begin{tabular}{c|c|ccccccc|cccccc}
\cline{1-15} 
\multirow{2}{*}{Application} & \multirow{2}{*}{Paper} & \multicolumn{9}{c|}{Reward} & \multicolumn{4}{c}{Algorithm} \\ \cline{3-15} 
 & & \rotatebox{90}{PnL} & \rotatebox{90}{Return} & \rotatebox{90}{VR} & \rotatebox{90}{IS} & \rotatebox{90}{Shaped reward} & \rotatebox{90}{Inventory Penalty} & \rotatebox{90}{Market Quality} & \rotatebox{90}{DQN} & \rotatebox{90}{PG} & \rotatebox{90}{PPO} & \rotatebox{90}{simulator} & \rotatebox{90}{TBD} & \rotatebox{90}{TBD} \\ \hline
\multirow{9}{*}{\rotatebox{90}{Portfolio Management}} 
& \cite{jiang2017deep} & & \cmark & & & & & & & & & \red{TBD} & & \\
 & \cite{yu2019model} & & \cmark & & & & & & & & & & & \\
 & \cite{zhang2020deep} & & \cmark & & & & & & & & & & & \\
 &\cite{ye2020reinforcement} & & & \cmark & & & & & & & & & & \\
 &\cite{nan2020sentiment} & & \cmark & & & & & & & & & & & \\
 &\cite{wang2021deeptrader} & & \cmark & & & & & & & & & & & \\
 & \cite{wang2021commission} & & \cmark & & & & & & & & & & & \\
 & \cite{benhamou2020aamdrl} & & \cmark & & & & & & & & & & & \\
& \cite{benhamou2021detecting} & & \cmark & & & & & & & & & & & \\ \cline{1-15} 
\multirow{8}{*}{\rotatebox{90}{Optimal Execution}} & 
\citet{nevmyvaka2006reinforcement} & \cmark & & & & & & & \cmark & & & & & \\
 & \citet{deng2016deep} & \cmark & & \cmark & & & & & & \cmark & & & & \\
 & \citet{wei2019model} &\cmark & & & & & & & & & & \cmark & & \\
 & \citet{lin2020E2E} & & & & \cmark & & & & & & \cmark & & & \\
 & \citet{fang2021universal} & & & & &\cmark & & & & & \cmark & & & \\
& \citet{lin2020deep} & & & & &\cmark & & & \cmark & & & & & \\
 & \citet{shen2014risk} & \cmark & & & & & & & \cmark & & & & & \\
 &\citet{hendricks2014reinforcement} & & & &\cmark & & & & \cmark & & & & & 
 \\\cline{1-15} 
\end{tabular}
\end{table}

==> Tables/table_optimal_execution.tex <==

% We introduce the following abbrevations. 
% For state, we use PA to denote Past Actions, Pos to denote the current Positions, xx. 
% For action, we use Qty to denote the quantity that we are going to place, Dir to denote the direction of this placement (negative or positive), and P to denote the price. 
% We use to emphasize it is discritized 

\begin{table}[t]
\caption{Literature on RL methods for Optimal Execution. 
}
\label{table:optimal_execution}
% 		\centering
% \hspace{-2cm}
% \small
% \renewcommand{\arraystretch}{1.5}
\begin{tabular}{m{2cm} llll}
    \hline
     Study & State & Action & Reward & Algorithm \\ %  & Data
\hline
%
   \citet{nevmyvaka2006reinforcement} & Inventory, Spread,  Time,  Volume
  &  bid price  &  PnL &  DQN \\ 
\hline
%
   \citet{deng2016deep} & Price  &  long/hold/short
  &\makecell{PnL \& VR}    & PG   \\ 
\hline
%
   \citet{wei2019model} & Inventory,  E2E
  &  quantity  & PnL  & \makecell{Simulator \\ \& model-free}   \\ 
\hline
%
   \citet{lin2020E2E} & Inventory,  Time,  E2E
  &  quantity  & IS  & PPO   \\ 
\hline
%
   \citet{fang2021universal} &  Inventory,  Price,  Time,   Volume
 &  quantity  & shaped reward  & PPO  \\ 
\hline
%
   \citet{lin2020deep} & Inventory,  Price,  Spread,  Time,  E2E
  &  quantity  & shaped reward  &  DQN  \\ 
\hline
%
   \citet{shen2014risk} &  Inventory,  Spread 
 &  bid price
  & PnL  &  DQN \\ 
\hline
%
   \citet{hendricks2014reinforcement} & Inventory,  Spread,   Time,  Volume  & quantity  &  IS & DQN  \\ 
  \hline
\end{tabular}
\end{table}











% \begin{table}

% \begin{tabular}{ | m{2cm}  m{2.5cm} m{2.5cm}  m{2.5cm} m{1.7cm} m{2cm} | } 
%   \hline
%   Reference & State & Action & Reward & Algorithm & Data/Simulator \\ 
%   \hline
%   %
%    \citet{nevmyvaka2006reinforcement} &   &    &   &   & \\ 
%   \hline
%   %
%    \citet{deng2016deep} &   &    &   &   & \\ 
%   \hline
%   %
%   \citet{wei2019model} &   & Qty, Dir    &  delta of middle price $\times$  Qty & DDQN/PG/A2C & \\ 
%   \hline
%   %
%   \citet{roa2019towards} &   &    &   & existing IRL methods & \\ 
%   \hline
%   %
%   \citet{karpe2020multi} &   &  Qty, P (d)  & price slippage $\times$  Qty & DDQN & \\ 
%   \hline
%   %
%    \citet{fang2021universal}  &   &    &   &   & \\ 
%   \hline
% \end{tabular}
% % \end{table}




% "private states = (time remaining, quantity remaining)
% market state variables = (bid-ask spread, volume imbalance, one-period price return, t-period price return)"


% past actions + current positions + AutoEncoder(past observations)
